Nondeterministic Behaviours in Double Categorical Systems Theory

In this paper, we build double theories capturing the idea of nondeterministic behaviors and trajectories. Following Libkind and Myers' Double Operadic Theory of Systems, we construct monoidal semi double categories of interfaces, along with what we call semimodules of systems, in the case of Moore machines, working with Markov categories with conditionals to handle nondeterminism. We use conditional products in these Markov categories to define trajectories in a compositional way, and represent nondeterministic systems using Markov maps; channels between systems are assumed to be deterministic.

==> subs_arena_mealy_constr.tex <==
\subsection{The double category $Arena^{\mathrm{Mealy}}_{\CC}(\GG)$}\label{appendix_Arena_Mealy}


==> subs_knight.tex <==

\subsection{Knightian trajectories}\label{subsection_Knight}


Recall that the clock system is the trivial system, where $S=I= \Omega = O = *$. Now, let us consider for instance a system $(\Omega, {\begin{pmatrix} S \\ S  \\ \end{pmatrix}} \leftrightarrows {\begin{pmatrix} I \\ O  \\ \end{pmatrix}})$ where $\Omega = \lbrace 0, 1 \rbrace$. Then, the update function $update: \lbrace 0, 1 \rbrace \times S \times I \rightarrow S$ can be viewed as a \emph{deterministic update that depends on a nondeterministic binary choice}. A priori, this choice is Knightian, i.e. \emph{there is no prior on its distribution in the definition of the system}. However, any trajectory, i.e. morphism of systems from the clock to our system $S$, must specify a distribution on these binary choices: the Markov maps $s^n: * \rightarrow \Omega^{n+1} \times S^{n+1} \times I^{n+1}$ encode joint distributions on binary choices, states and inputs, all at once.


Let us now explain how one can represent systems with probabilistic updates, e.g. Markov chains. The idea is to add sources of randomness to the space $\Omega$, then make sure to only consider trajectories where the marginals on $\Omega$ have suitable laws. For instance, given a (closed) Markov chain on the discrete countable set $\mathbb{N}$, one can define, for each $n$, a partition of $(0,1)$ into intervals $I_{m,n}$, $m \in \mathbb{N}$, such that $I{m,n}$ is of length $p(m | n)$, for all $m, n$. Then, consider the standard Borel space $\Omega = {(0,1)}^{\mathbb{N}}$ and the measurable map $update: \mathbb{N}  \rightarrow \mathbb{N}$ defined by $update(n, (\omega_i)_i) = m$ when $\omega_n \in I_{m,n}$. Then, one can check that, for all $n$, the pushforward measure $update_*(\lambda^{\otimes \mathbb{N}} \otimes \delta_n)$ is equal to the probability measure $p( \cdot | n)$, where $\lambda$ denotes the uniform distribution on $(0, 1)$. In fact, this \emph{ad hoc} example can be generalized.


First, let us recall a few facts on cumulative distribution functions.

\begin{definition}
Let $X$ be a real-valued random variable. Let $F_X: \mathbb{R} \rightarrow [0, 1]$ be defined by $F_X(t) = P(X \leq t)$ for all $t$. It is the \emph{cumulative distribution function} of $X$. 


Then, the \emph{inverse distribution function} of $X$, or \emph{quantile function}, often denoted $F_X^{-1}: (0, 1) \rightarrow \mathbb{R}$, is defined by $F_X^{-1}(p) = \inf \lbrace t \in \mathbb{R} \, | \, F_X(t) \geq p \rbrace$.

	
\end{definition}


Note that the function $F_X$ only depends on the law of $X$; actually, $F_X$ is a complete invariant for the law of $X$. 


\begin{fact}\label{fact_quantile_functions}
	For all real-valued random variables $X$, the function $F_X^{-1}$ satisfies the following properties:
	
	\begin{enumerate}
		\item For all $p \in (0, 1)$, for all $t \in \mathbb{R}$, we have $F_X(t) \geq u$ if and only if $t \geq F_X^{-1}(p)$.
		\item The pushforward distribution $G_*(\lambda)$ is the law of $X$, where $\lambda$ is the uniform measure on $(0, 1)$.
	\end{enumerate}
	
\end{fact}
	



\begin{prop}\label{prop_uniformization}
	Let $S$, $I$ be standard Borel spaces, and $f: S \times I \rightarrow S$ be a measurable Markov kernel, i.e. a morphism in BorelStoch. Then, there exists a measurable function $G: (0, 1) \times S \times I \rightarrow S$ such that, for all $(s,i) \in S \times I$, the pushforward measure $G_*(\lambda \otimes \delta_s \otimes \delta_i)$ is equal to $f(s,i)$.
\end{prop}

\begin{proof}
This is the content of Lemma 3.22 in \cite{Kall-Proba-book}. We recall the proof for completeness. The idea is to use cumulative distribution functions to generate randomness uniformly. Choose a bimeasurable isomorphism $\iota: S \simeq \mathbb{R}$, $S \simeq \mathbb{N}$ or $S \simeq \lbrace 1, \ldots, n \rbrace$, so that it suffices to deal with the cases of $\mathbb{R}$, $\mathbb{N}$ and $\lbrace 1, \ldots, n \rbrace$. We shall deal with the case $S \simeq \mathbb{R}$, leaving the rest to the reader.

Then, consider the measurable Markov kernel $f^{'} := (f; \iota): S \times I \rightarrow \mathbb{R}$. Let $G: (0, 1) \times S \times I \rightarrow S$ be defined by $G(p, s, i) = \iota^{-1}(F_{f^{'}(s, i)}^{-1}(p))$. Then, by Fact \ref{fact_quantile_functions} above, we know that, for all $s, i$, the pushforward measure $G_*(\lambda \otimes \delta_s \otimes \delta_i)$ is equal to $f(s,i)$.

\begin{claim}
	The function $G: (0, 1) \times S \times I \rightarrow S$ is measurable. 
\end{claim} 

\begin{proof}{Proof of the Claim}
	Since $\iota$ is a bimeasurable isomorphism, it is equivalent to show that the function $G_1 := \iota \circ G: (0, 1) \times S \times I \rightarrow \mathbb{R}$ is measurable. By Fact \ref{fact_quantile_functions}, we have, for all $t \in \mathbb{R}$, for all $(p, s, i) \in (0, 1) \times S \times I$, $G_1(p, s, i) \leq t$ if and only if $p \leq F_{f^{'}(s,i)}(t)$, if and only if $\mathbb{P}(f^{'}(s,i) \geq t) \geq p$. Thus, fixing $t$, we have $G_1^{-1}((-\infty, t]) = \lbrace (p, s, i) \in (0,1) \times S \times I \, | \, \mathbb{P}(\iota(f(s,i)) \geq t) \geq p \rbrace$, where $G_1^{-1}((-\infty, t])$ denotes the preimage of the interval $(-\infty, t]$ by the function $G_1$. Since $f: S \times I \rightarrow S$ is a measurable Markov kernel, the right hand side of the equation is a measurable set. Thus, we have proved that the preimage $G_1^{-1}((-\infty, t])$ is measurable for all $t$. This implies that the map $G_1$ is measurable. 
\end{proof}

This concludes the proof.
\end{proof}

\begin{remark}
	\begin{enumerate}
		\item One would like the construction done in Proposition \ref{prop_uniformization} to be functorial, i.e. compatible with composition of measurable Markov kernels. We leave this to future work.
		
		\item Constraining trajectories of systems to have prescribed marginals on $\Omega$, in a clear and abstract way, would be of interest.
	\end{enumerate}

\end{remark}






In our formalism, one can define simple systems that represent Knightian choices. 


\begin{itemize}
	\item For any standard Borel space $\Omega_0$, define the system $Knight_{\Omega_0} = (\Omega_0, {\begin{pmatrix} * \\ *  \\ \end{pmatrix}} \leftrightarrows {\begin{pmatrix} * \\ *  \\ \end{pmatrix}})$ given by the unique maps $update: \Omega_0 \times * \times * \rightarrow *$ and $expose: * \rightarrow *$. This system can be viewed as one that only makes Knightian choices of type $\Omega_0$, and does nothing else, not even storing them in its state.


Then, a morphism of systems from $Knight_{\Omega_0}$ to a system $(\Omega, {\begin{pmatrix} S \\ S  \\ \end{pmatrix}} \leftrightarrows {\begin{pmatrix} I \\ O  \\ \end{pmatrix}})$ is given by Markov maps $s^n: {\Omega_0}^{n+1} \rightarrow \Omega^{n+1} \times S^{n+1} \times I^{n+1}$, $p^n: * \rightarrow I^{n+1} \times O^{n+1}$ and $\phi^n: * \rightarrow S^{n+1}$, with some compatibility conditions. In other words, such a $Knight_{\Omega_0}$-behavior essentially amounts to \emph{families of trajectories parametrized by lists of Knightian choices} in $\Omega_0$: given such a $Knight_{\Omega_0}$-behavior, each sequence $u \in {\Omega_0}^{\mathbb{N}}$ yields a probabilistic trajectory of the system $(\Omega, {\begin{pmatrix} S \\ S  \\ \end{pmatrix}} \leftrightarrows {\begin{pmatrix} I \\ O  \\ \end{pmatrix}})$, in the previous sense.



A simple class of behaviors is made of those that satisfy the following conditions:

\begin{itemize}
	\item We have $\Omega = \Omega_0$.
	\item The marginals $(s^n; \pi) : {\Omega_0}^{n+1} \rightarrow S^{n+1} \times I^{n+1}$ are constant probability distributions that do not depend on the argument in ${\Omega_0}^{n+1}$.
	\item The composite $(s^n ; \pi): {\Omega_0}^{n+1} \rightarrow \Omega^{n+1}$ is the identity of ${\Omega_0}^{n+1}$ for all $n$.
\end{itemize}
Such a behavior corresponds to having only prescribed joint probability distributions for states and inputs that do not depend in the choices in $\Omega_0$, and leaving the nondeterministic choices unspecified.





Now, using $x$-composition of squares in $ArenaSys^{\mathrm{Moore}}_{\CC}(\GG)$, if one is given a probabilistic trajectory of the system $Knight_{\Omega_0}$ and a $Knight_{\Omega_0}$-behavior of the system $(\Omega, {\begin{pmatrix} S \\ S  \\ \end{pmatrix}} \leftrightarrows {\begin{pmatrix} I \\ O  \\ \end{pmatrix}})$, one gets a probabilistic trajectory of the system $(\Omega, {\begin{pmatrix} S \\ S  \\ \end{pmatrix}} \leftrightarrows {\begin{pmatrix} I \\ O  \\ \end{pmatrix}})$. 




%
%Consider the following model for epidemiology: 
%
%\begin{itemize}
%	\item 
%\end{itemize}


\item If one wants to allow for the states, inputs and outputs to depend on Knightian choices, one can consider more sophisticated systems, as follows:


Let $\Omega_0$, $\Omega_1$, $\Omega_2$, be standard Borel spaces, and define the system $(\Omega_0 \times \Omega_1, {\begin{pmatrix} \Omega_1 \times \Omega_2 \\  \Omega_1\times \Omega_2 \\ \end{pmatrix}} \leftrightarrows {\begin{pmatrix} \Omega_2 \\ \Omega_1  \\ \end{pmatrix}})$, whose output map is the identity of $\Omega_1$, and where the map $update: \Omega_0 \times \Omega_1 \times S \times I \rightarrow S$ is given by $update(\omega_0, \omega_1, s, i) = (\omega_1, i) \in \Omega_{1} \times \Omega_{2} = S$.  

\end{itemize}

\begin{remark}
	If one wishes to study imprecise probability behaviors where the number of Knightian choices does not grow linearly with time, one can use more general systems than the simple ones we described here.
\end{remark}


==> subs_mealy_thm.tex <==
\subsection{A variant for Mealy machines: the virtual double theory $T^{\mathrm{Mealy}}(\CC, \GG)$}

Here, we define another systems theory $T^{\mathrm{Mealy}}(\CC, \GG)$, given a Directed Acyclic Graph $\GG$ and a Markov category with conditionals $\CC$. It shall be based on Mealy machines rather than Moore machines. Recall that such systems, in their basic form, are given by maps $S \otimes I \rightarrow S \otimes O$ in symmetric monoidal categories, where $S$, $I$, $O$ denote the state space, the input space, and the output space respectively.

Taking inspiration from monoidal streams, we use the following notion for systems:

\begin{definition}\label{defi_G-Mealy}
	The symmetric monoidal category $Mealy_{\CC}(\GG)$ of $\GG$-indexed Mealy machines is defined as follows:
	\begin{itemize}
		\item The objects are the functors from $\GG^{op}$ to $\CC_{det}$. In other words, an object $A \in Mealy_{\CC}(\GG)$ is given by a collection of objects $A(a) \in \CC$, for $a \in \GG$, and deterministic restriction morphisms $res: A(b) \rightarrow A(a)$ in $\CC_{det}$, for all edges $a \rightarrow b$ in $\GG$.
		\item A morphism $A \rightarrow B$ is given by an object $S \in Mealy_{\CC}(\GG)$, along with morphisms $f_{a\rightarrow b}: A(b) \otimes S(a) \rightarrow B(b) \otimes S(b)$ in $\CC$, for all edges $a \rightarrow b$ in $\GG$, with the following condition: 
		
		 For all edges $a \rightarrow b$, the following diagram commutes in $\CC$:
			% https://q.uiver.app/#q=WzAsNCxbMCwwLCJBKGIpIFxcb3RpbWVzIFMoYSkiXSxbMCwyLCJCKGIpIFxcb3RpbWVzIFMoYikiXSxbMSwyLCJTKGIpIl0sWzIsMiwiUyhhKSJdLFswLDMsIlxccGkiXSxbMiwzLCJyZXMiLDJdLFsxLDIsIlxccGkiLDJdLFswLDEsImZfe2FcXHJpZ2h0YXJyb3cgYn0iLDJdXQ==
\[\begin{tikzcd}
	{A(b) \otimes S(a)} \\
	\\
	{B(b) \otimes S(b)} & {S(b)} & {S(a)}
	\arrow["{f_{a\rightarrow b}}"', from=1-1, to=3-1]
	\arrow["\pi", from=1-1, to=3-3]
	\arrow["\pi"', from=3-1, to=3-2]
	\arrow["res"', from=3-2, to=3-3]
\end{tikzcd}\]

		We may denote such a morphism $A \xrightarrow[S]{} B$.

		\item Sequential composition is defined as follows: let $f: A \xrightarrow[S]{} B$ and $g: B \xrightarrow[T]{} C$ be morphisms. The formula is the following, for all $a \rightarrow b$: ${(f;g)}_{a \rightarrow b} = f_{a \rightarrow b} \otimes T(a) ; \sigma_{S(b) , T(a)} ; g_{a \rightarrow b} \otimes S(b) ; \sigma(T(b), S(b))$, as morphisms in $\CC$ of type  $A(b) \otimes S(a) \otimes T(a) \rightarrow C(b) \otimes S(b) \otimes T(b)$.
		
		% Their composite $f; g: A \xrightarrow[S \otimes T] C$ is given by the composites $A(b) \otimes S(a) \otimes T(a) \xrightarrow{f_{a \rightarrow b} \otimes T(a)} B(b) \otimes S(b) \otimes T(a) \xrightarrow{\sigma} B(b) \otimes T(a) \otimes S(b) \xrightarrow{g_{a \rightarrow b} \otimes S(b)} C(b) \otimes T(b) \otimes S(b) \xrightarrow[]{\sigma} C(b) \otimes S(b) \otimes T(b)$, for all $a \rightarrow b$.
		
% https://q.uiver.app/#q=WzAsNSxbMCwwLCJBKGIpIFxcb3RpbWVzIFMoYSkgXFxvdGltZXMgVChhKSJdLFsxLDAsIkIoYikgXFxvdGltZXMgUyhiKSBcXG90aW1lcyBUKGEpIl0sWzIsMCwiQihiKSBcXG90aW1lcyBUKGEpIFxcb3RpbWVzIFMoYikiXSxbMywwLCJDKGIpIFxcb3RpbWVzIFQoYikgXFxvdGltZXMgUyhiKSJdLFs0LDAsIkMoYikgXFxvdGltZXMgUyhiKSBcXG90aW1lcyBUKGIpIl0sWzAsMSwiZl97YSBcXHJpZ2h0YXJyb3cgYn0gXFxvdGltZXMgVChhKSJdLFsxLDIsIlxcc2lnbWEiXSxbMiwzLCJnX3thIFxccmlnaHRhcnJvdyBifSJdLFszLDQsIlxcc2lnbWEiXV0=
% \[\begin{tikzcd}
% 	{A(b) \otimes S(a) \otimes T(a)} & {B(b) \otimes S(b) \otimes T(a)} & {B(b) \otimes T(a) \otimes S(b)} & {C(b) \otimes T(b) \otimes S(b)} & {C(b) \otimes S(b) \otimes T(b)}
% 	\arrow["{f_{a \rightarrow b} \otimes T(a)}", from=1-1, to=1-2]
% 	\arrow["\sigma", from=1-2, to=1-3]
% 	\arrow["{g_{a \rightarrow b}}", from=1-3, to=1-4]
% 	\arrow["\sigma", from=1-4, to=1-5]
% \end{tikzcd}\]

		\item Parallel composition of morphisms, and more generally the symmetric monoidal structure of $Mealy_{\CC}(\GG)$, is defined using that of $\CC$.

	\end{itemize}
\end{definition}

\begin{remark}
	For the definition above, we only need the symmetric monoidal structure of $\CC$. The fact that $\CC$ is a Markov category with conditionals shall be used when defining the virtual (oplax) double category structure.
\end{remark}



Now, since we are also interested in imprecise probability and Knightian choices, we shall consider \emph{parametric} $\GG$-indexed Mealy machines.

\begin{definition}\label{defi_Para_Mealy}
	The symmetric monoidal category $ParaMealy_{\CC}(\GG)$ of \emph{parametric} $\GG$-indexed Mealy machines has the same objects as $Mealy_{\CC}(\GG)$, and morphisms $A \rightarrow B$ are given by pairs $(S, \Omega)$ of objects of $ParaMealy_{\CC}(\GG)$, along with maps $f_{a \rightarrow b}: A(b) \otimes \Omega(b) \otimes S(a) \rightarrow B(b) \otimes S(b)$, for all edges $a \rightarrow b$, such that the diagrams below commute:

	% https://q.uiver.app/#q=WzAsNCxbMCwwLCJBKGIpIFxcb3RpbWVzIFxcT21lZ2EoYikgXFxvdGltZXMgIFMoYSkiXSxbMCwyLCJCKGIpIFxcb3RpbWVzIFMoYikiXSxbMSwyLCJTKGIpIl0sWzIsMiwiUyhhKSJdLFswLDMsIlxccGkiXSxbMiwzLCJyZXMiLDJdLFsxLDIsIlxccGkiLDJdLFswLDEsImZfe2FcXHJpZ2h0YXJyb3cgYn0iLDJdXQ==
\[\begin{tikzcd}
	{A(b) \otimes \Omega(b) \otimes  S(a)} \\
	\\
	{B(b) \otimes S(b)} & {S(b)} & {S(a)}
	\arrow["{f_{a\rightarrow b}}"', from=1-1, to=3-1]
	\arrow["\pi", from=1-1, to=3-3]
	\arrow["\pi"', from=3-1, to=3-2]
	\arrow["res"', from=3-2, to=3-3]
\end{tikzcd}\]

% https://q.uiver.app/#q=WzAsNCxbMiwwLCJBKGIpIFxcb3RpbWVzXFxPbWVnYShiKSBcXG90aW1lcyBTKGEpIl0sWzAsMCwiQShjKVxcb3RpbWVzIFxcT21lZ2EoYykgXFxvdGltZXMgUyhiKSJdLFswLDIsIkIoYykgXFxvdGltZXMgUyhjKSJdLFsyLDIsIkIoYikgXFxvdGltZXMgUyhiKSJdLFsxLDAsInJlcyBcXG90aW1lcyByZXMgXFxvdGltZXMgcmVzIl0sWzIsMywicmVzIFxcb3RpbWVzIHJlcyJdLFsxLDIsImZfe2IgXFxyaWdodGFycm93IGN9IiwxXSxbMCwzLCJmX3thIFxccmlnaHRhcnJvdyBifSIsMV1d
\[\begin{tikzcd}
	{A(c)\otimes \Omega(c) \otimes S(b)} && {A(b) \otimes\Omega(b) \otimes S(a)} \\
	\\
	{B(c) \otimes S(c)} && {B(b) \otimes S(b)}
	\arrow["{res \otimes res \otimes res}", from=1-1, to=1-3]
	\arrow["{f_{b \rightarrow c}}"{description}, from=1-1, to=3-1]
	\arrow["{f_{a \rightarrow b}}"{description}, from=1-3, to=3-3]
	\arrow["{res \otimes res}", from=3-1, to=3-3]
\end{tikzcd}\]



The structure of a symmetric monoidal category for $ParaMealy_{\CC}(\GG)$ is defined in a way similar to $Mealy_{\CC}(\GG)$; let us note that morphisms $A \xrightarrow[S, \Omega] B$ and $B \xrightarrow[T, \Omega'] C$ compose into $A \xrightarrow[S  \otimes T, \Omega \otimes \Omega'] C$.

\end{definition}

\begin{theorem}\label{theo_Mealy_main}
	There exists a systems theory $T^{\mathrm{Mealy}}(\CC, \GG)$, whose symmetric monoidal category of systems is (isomorphic to) $ParaMealy_{\CC}(\GG)$.
\end{theorem}



Let us now sketch the proof of Theorem \ref{theo_Mealy_main}, by constructing the systems theory $T^{\mathrm{Mealy}}(\CC, \GG)$. The ideas are similar, \emph{mutatis mutandis}, to the case of Moore machines. The details can be found in Appendix \ref{appendix_Arena_Mealy} and \ref{appendix_ArenaSys_Mealy}.


\begin{construction}\label{constr_Arena_Mealy_C^G}
	We construct an oplax virtual double category $ArenaSys^{\mathrm{Mealy}}_{\CC}(\GG)$ with a (virtual) double functor $H: ArenaSys^{\mathrm{Mealy}}_{\CC}(\GG) \rightarrow y(2)$, as follows:
	
	\begin{enumerate}
		\item The objects are functors $\GG^{op} \rightarrow \CC_{det}$.
		\item The $1$-category $H^{-1}(0)_y \subseteq {ArenaSys^{\mathrm{Mealy}}_{\CC}(\GG)}_y$ is $ParaMealy_{\CC}(\GG)$.

		\item The $1$-category $H^{-1}(1)_y \subseteq {ArenaSys^{\mathrm{Mealy}}_{\CC}(\GG)}_y$ is $ParaMealy_{\CC_{det}}(\GG)$. In other words, lenses are \emph{deterministic} parametric $\GG$-indexed Mealy machines. 

		\item Morphisms in $H^{-1}(0 \rightarrow 1)_y$ are the same as those in $H^{-1}(0)_y$, i.e. (possibly nondeterministic) parametric $\GG$-indexed Mealy machines.  
		
		
		\item Horizontal morphisms $A \rightarrow B$, or $x$-morphisms, are natural transformations, i.e. morphisms in $[\GG^{op}; \CC]$. Note that, although the restriction maps defining $A$ and $B$ are deterministic, the maps involved in the $x$-morphisms need not be so. Such $x$-morphisms either belong to $H^{-1}(0)$ or to $H^{-1}(1)$.
		
		
		
		\item Just like $x$-morphisms, the $2$-cells are defined uniformly across the fibers $H^{-1}(0)$, $H^{-1}(1)$, and $H^{-1}(0 \rightarrow 1)$. A $2$-cell $s$ with the following boundary:

% https://q.uiver.app/#q=WzAsNyxbMCwwLCJBXzEiXSxbMCw0LCJBXzIiXSxbNCwwLCJCXzEiXSxbNCwxLCJCXzIiXSxbNCw0LCJCX24iXSxbNCwzLCJCX3tuLTF9Il0sWzQsMiwiXFx2ZG90cyJdLFsyLDMsIlRfMSwgXFxPbWVnYV8xIl0sWzUsNCwiVF97bi0xfSwgXFxPbWVnYV97bi0xfSJdLFsxLDRdLFswLDJdLFszLDZdLFs2LDVdLFswLDEsIlMsIFxcT21lZ2EiXV0=
\[\begin{tikzcd}
	{A_1} &&&& {B_1} \\
	&&&& {B_2} \\
	&&&& \vdots \\
	&&&& {B_{n-1}} \\
	{A_2} &&&& {B_n}
	\arrow[from=1-1, to=1-5]
	\arrow["{S, \Omega}", from=1-1, to=5-1]
	\arrow["{T_1, \Omega_1}", from=1-5, to=2-5]
	\arrow[from=2-5, to=3-5]
	\arrow[from=3-5, to=4-5]
	\arrow["{T_{n-1}, \Omega_{n-1}}", from=4-5, to=5-5]
	\arrow[from=5-1, to=5-5]
\end{tikzcd}\]


		is given by a collection of morphisms $s_{a \rightarrow b}$ in $\CC$, of type $A_1(b) \otimes \Omega(b) \otimes S(a) \rightarrow B_1(b) \otimes (\bigotimes_{i=1}^{n-1} T_i(b) \otimes \Omega_i(b) \otimes B_{i+1}(b))$, that satisfy some compatibility conditions.
		
Composition of these $2$-cells is defined using the conditional products in $\CC$, and yields an oplax virtual double category. In the fiber $H^{-1}(0) = Arena^{\mathrm{Mealy}}_{\CC}(\GG)$, i.e. with deterministic $y$-morphisms, this structure comes from a genuine (strict) double category.

	\end{enumerate}	
\end{construction}

